Creating ConLangs to Probe the Metalinguistic Grammatical Knowledge of LLMs

We present a system that uses LLMs as a tool in the development of Constructed Languages -- ConLangs, which we call IASC (Interactive Agentic System for ConLangs). The system is modular in that it creates each of the components -- phonology, morphology and syntax, lexicon, orthography, and grammatical handbook, using module-specific sets of prompts. The approach is agentic in that various modules allow for refining the output given automatically-generated commentary on a previous step. Our main goals are twofold. First, we aim to provide tools that facilitate an engaging and enjoyable experience in creating artificially constructed languages. Second, the focus of this paper is on using our ConLang framework as a novel way to explore what LLMs 'know' about language -- not what they know about any particular language or encyclopedic facts, but how much they know about and understand language and linguistic concepts. In the experiments, we particularly focus on the morphosyntax module and show that there is a fairly wide gulf in capabilities both among different LLMs and among different linguistic specifications, with it being notably easier for systems to deal with more typologically common patterns than rarer ones. All code is released.

==> Tables/morph-full-results.tex <==
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \scriptsize
    \begin{tabular}{@{}llrrrrrrrrr@{}} \toprule
Model & Language & BLEU & ChrF++ & WER & CER & TER & SER & MFER & MSER & LemF1 \\
\midrule
gpt-4o-mini & arabic & 0.19 & 10.49 & 106.38 & 70.83 & 90.60 & 77.05 & 73.20 & 75.13 & 53.46 \\
 & fijian & 0.28 & 10.51 & 88.42 & 62.49 & 63.56 & 62.07 & 57.52 & 60.24 & 43.51 \\
 & french & 0.20 & 12.58 & 86.85 & 65.09 & 73.97 & 45.15 & 64.26 & 54.71 & 56.77 \\
 & hixkaryana & 0.30 & 11.93 & 118.68 & 85.15 & 65.93 & 67.16 & 61.43 & 64.30 & 34.94 \\
 & mizo & 0.27 & 11.14 & 99.07 & 79.94 & 69.88 & 51.53 & 59.12 & 55.32 & 53.92 \\
 & turkish & 0.20 & 12.72 & 124.06 & 78.73 & 101.50 & 67.67 & 71.74 & 69.71 & 51.97 \\
 & vietnamese & 0.33 & 12.62 & 79.12 & 42.10 & 75.76 & 62.72 & 54.82 & 58.77 & 50.25 \\
 & welsh & 0.21 & 10.54 & 86.71 & 60.50 & 78.03 & 61.02 & 60.31 & 60.66 & 53.88 \\
 & hard & 0.18 & 12.08 & 134.19 & 79.69 & 115.81 & 82.72 & 82.44 & 82.58 & 48.55 \\ \cmidrule{2-11}
 & Average & 0.24 & 11.62 & 102.51 & 69.35 & 81.67 & 64.12 & 64.98 & 64.55 & 38.47 \\
\midrule
gpt-5-mini & arabic & 0.17 & 5.07 & 74.16 & 35.94 & 60.40 & 15.41 & 36.71 & 26.06 & 84.11 \\
 & fijian & 0.19 & 7.17 & 101.69 & 79.42 & 76.27 & 93.10 & 66.19 & 79.65 & 39.49 \\
 & french & 0.12 & 5.61 & 55.34 & 32.71 & 61.64 & 30.10 & 27.18 & 28.64 & 91.26 \\
 & hixkaryana & 0.21 & 7.36 & 93.41 & 52.45 & 82.42 & 50.37 & 48.44 & 49.40 & 76.04 \\
 & mizo & 0.17 & 8.89 & 146.89 & 88.87 & 139.75 & 103.05 & 70.82 & 86.94 & 49.15 \\
 & turkish & 0.18 & 6.05 & 103.76 & 62.00 & 118.42 & 101.50 & 52.97 & 77.24 & 77.95 \\
 & vietnamese & 0.32 & 12.26 & 66.33 & 38.73 & 75.76 & 78.40 & 49.21 & 63.81 & 57.10 \\
 & welsh & 0.21 & 7.44 & 45.09 & 27.46 & 52.02 & 15.25 & 25.24 & 20.25 & 87.64 \\
 & hard & 0.16 & 4.60 & 126.84 & 76.22 & 115.81 & 66.18 & 76.06 & 71.12 & 59.52 \\
\cmidrule{2-11}
 & Average & 0.19 & 7.16 & 90.39 & 54.87 & 86.94 & 61.49 & 50.31 & 55.90 & 69.14 \\
\midrule
gpt-5 & arabic & 0.20 & 5.47 & 62.42 & 39.04 & 60.40 & 15.41 & 33.23 & 24.32 & 90.27 \\
 & fijian & 0.20 & 6.54 & 70.62 & 80.61 & 50.85 & 93.10 & 46.90 & 70.00 & 56.28 \\
 & french & 0.15 & 4.92 & 83.29 & 53.25 & 73.97 & 15.05 & 40.39 & 27.72 & 79.41 \\
 & hixkaryana & 0.21 & 7.57 & 67.03 & 32.52 & 65.93 & 33.58 & 38.42 & 36.00 & 79.78 \\
 & mizo & 0.17 & 9.01 & 165.84 & 96.47 & 153.73 & 137.40 & 77.69 & 107.55 & 36.10 \\
 & turkish & 0.19 & 5.01 & 123.31 & 80.62 & 152.26 & 118.42 & 79.59 & 99.00 & 66.13 \\
 & vietnamese & 0.31 & 12.57 & 64.98 & 39.18 & 60.61 & 62.72 & 47.07 & 54.90 & 58.40 \\
 & welsh & 0.19 & 7.55 & 40.17 & 25.74 & 52.02 & 15.25 & 20.27 & 17.76 & 88.17 \\
 & hard & 0.17 & 5.20 & 125.37 & 71.26 & 115.81 & 49.63 & 74.09 & 61.86 & 59.52 \\
\cmidrule{2-11}
 & Average & 0.20 & 7.09 & 89.23 & 57.63 & 87.29 & 60.06 & 50.85 & 55.46 & 68.23 \\
\midrule
gemini-2.5-flash & arabic & 0.00 & 7.29 & 66.11 & 37.37 & 60.40 & 0.00 & 39.50 & 19.75 & 88.41 \\
 & fijian & 0.19 & 10.12 & 92.09 & 59.29 & 63.56 & 46.55 & 56.77 & 51.86 & 59.68 \\
 & french & 0.13 & 6.83 & 73.70 & 44.05 & 73.97 & 15.05 & 42.09 & 28.57 & 82.13 \\
 & hixkaryana & 0.19 & 8.45 & 98.17 & 54.53 & 115.38 & 50.37 & 60.00 & 55.18 & 65.18 \\
 & mizo & 0.18 & 9.48 & 121.12 & 74.64 & 125.78 & 17.18 & 65.68 & 41.43 & 62.86 \\
 & turkish & 0.21 & 9.67 & 104.51 & 60.02 & 118.42 & 67.67 & 59.47 & 63.57 & 77.53 \\
 & vietnamese & 0.28 & 12.13 & 67.68 & 47.54 & 45.45 & 47.04 & 48.88 & 47.96 & 55.33 \\
 & welsh & 0.17 & 7.84 & 67.05 & 37.10 & 78.03 & 30.51 & 38.53 & 34.52 & 81.63 \\
 & hard & 0.10 & 4.27 & 125.74 & 85.88 & 115.81 & 115.81 & 83.81 & 99.81 & 49.19 \\ \cmidrule{2-11}
 & Average & 0.16 & 8.45 & 90.65 & 55.56 & 87.12 & 41.63 & 54.97 & 48.30 & 69.11 \\
\midrule
gemini-2.5-pro & arabic & 0.21 & 5.57 & 51.34 & 31.38 & 45.30 & 15.41 & 32.01 & 23.71 & 92.68 \\
 & fijian & 0.18 & 7.30 & 77.12 & 64.41 & 50.85 & 62.07 & 47.08 & 54.58 & 63.79 \\
 & french & 0.14 & 8.04 & 57.53 & 27.95 & 61.64 & 0.00 & 37.85 & 18.93 & 81.56 \\
 & hixkaryana & 0.22 & 8.89 & 98.90 & 44.01 & 131.87 & 50.37 & 55.74 & 53.06 & 69.78 \\
 & mizo & 0.15 & 8.02 & 177.33 & 107.35 & 125.78 & 68.70 & 76.31 & 72.51 & 41.82 \\
 & turkish & 0.18 & 7.34 & 110.15 & 53.85 & 135.34 & 67.67 & 57.71 & 62.69 & 79.65 \\
 & vietnamese & 0.31 & 12.87 & 49.83 & 31.41 & 30.30 & 31.36 & 35.57 & 33.46 & 73.16 \\
 & welsh & 0.18 & 9.87 & 47.98 & 26.82 & 65.03 & 15.25 & 29.06 & 22.16 & 88.48 \\
 & hard & 0.25 & 4.97 & 100.74 & 78.35 & 115.81 & 314.34 & 83.33 & 198.83 & 32.87 \\ \cmidrule{2-11}
 & Average & 0.20 & 8.10 & 85.66 & 51.73 & 84.66 & 69.46 & 50.52 & 59.99 & 69.31 \\
\midrule
claude-sonnet-3.5 & arabic & 0.00 & 5.67 & 68.12 & 36.08 & 60.40 & 0.00 & 41.57 & 20.78 & 91.62 \\
 & fijian & 0.15 & 6.96 & 139.55 & 118.16 & 152.54 & 108.62 & 72.68 & 91.05 & 41.16 \\
 & french & 0.15 & 6.23 & 64.93 & 33.37 & 86.30 & 15.05 & 40.75 & 27.90 & 79.93 \\
 & hixkaryana & 0.20 & 7.71 & 107.33 & 70.04 & 98.90 & 50.37 & 53.62 & 52.00 & 73.44 \\
 & mizo & 0.13 & 9.11 & 115.22 & 86.34 & 125.78 & 51.53 & 63.69 & 57.61 & 58.93 \\
 & turkish & 0.00 & 7.54 & 62.78 & 32.67 & 101.50 & 50.75 & 42.58 & 46.66 & 84.81 \\
 & vietnamese & 0.30 & 13.34 & 76.43 & 41.77 & 90.91 & 47.04 & 53.17 & 50.10 & 52.80 \\
 & welsh & 0.17 & 7.50 & 28.03 & 19.45 & 65.03 & 30.51 & 18.01 & 24.26 & 90.36 \\
 & hard & 0.15 & 4.85 & 115.81 & 73.07 & 99.26 & 49.63 & 73.06 & 61.35 & 66.11 \\ \cmidrule{2-11}
 & Average & 0.14 & 7.66 & 86.34 & 56.67 & 96.44 & 43.11 & 51.02 & 47.06 & 71.02 \\
\bottomrule
\end{tabular}
    \caption{Full results of the Morphosyntax module.}
    \label{tab:full-results}
\end{table*}

==> Tables/morph-metrics.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lp{20em}} \toprule
        Metric & Description \\ \midrule
        Translation Edit Rate \citep{Snover:EtAl:06} & Count of the edit operations from the hypothesis to the reference. \\
        BLEU \citep{Papineni:EtAl:02} & The average of the $n$-gram precisions ($n = 1, 2, 3, 4$) with a brevity penalty. \\
        ChrF++ \citep{Popovic:17} & The average of the character-level 6-gram F1 score and the word-level 2-gram F1 score. \\
        \midrule
        Stem Edit Rate (SER) & TER applied to the stems. That is, this metric only focuses on the overall word order and ignores specific morphological features attached to the stem. \\
        Morphological Feature Error Rate (MFER) & The average feature errors, grouped by prefixes and suffixes. \\
        Morphosyntactic Error Rate (MSER) & The (weighted) average of Stem Edit Rate and Morphological Feature Error Rate. \\
        Lemma F1 (LemF1) & The F1 score based on the lemmata of the predicted output. \\
        \bottomrule
    \end{tabular}
    \caption{List of the metrics.
    The metrics in the top half are existing metrics used in the previous literature.
    Those in the bottom half are newly proposed metrics used in this study.}
    \label{tab:metrics}
\end{table*}
